The INTERSPEECH 2021 Computational Paralinguistics Challenge: COVID-19 Cough, COVID-19 Speech, Escalation & Primates

The INTERSPEECH 2021 Computational Paralinguistics Challenge addresses four different problems for the first time in a research competition under well-defined conditions: In the COVID-19 Cough and COVID-19 Speech Sub-Challenges, a binary classification on COVID-19 infection has to be made based on coughing sounds and speech; in the Escalation SubChallenge, a three-way assessment of the level of escalation in a dialogue is featured; and in the Primates Sub-Challenge, four species vs background need to be classified. We describe the Sub-Challenges, baseline feature extraction, and classifiers based on the 'usual' COMPARE and BoAW features as well as deep unsupervised representation learning using the AuDeep toolkit, and deep feature extraction from pre-trained CNNs using the Deep Spectrum toolkit; in addition, we add deep end-to-end sequential modelling, and partially linguistic analysis.

==> temp_tables.tex <==
% tmp table 2d
\begin{table*}[t!]
 	\caption{
 	Results for the three Sub-Challenges. 
	%	The best results for test   (official baselines) for each Sub-Challenge are highlighted in bold.
		The \textbf{official baselines} for Test
%        which correspond to the best results obtained for development  
       are highlighted (bold and greyscale); 
        there are \textbf{no} official baselines for Dev.
        %Dev: Development.
      	$C$: Complexity parameter of the SVM/SVR, optimised for all from $10^{-5}$ to $1$.
        $N$: Codebook size for Bag-of-Audio-Words (BoAW) splitting the input into two codebooks (\textsc{ComParE}-LLDs/\textsc{ComParE}-LLD-deltas) of the same given size, with 50 assignments per frame. 
        $DenseNet121$: pre-trained CNN used for extraction of \ds{} features.
%        $S2SAE$: Sequence to Sequence Autoencoder. 
        $X$: Threshold power levels for  $S2SAE$ under which was clipped.
        \textsc{DiFE}: Lingustic feature extraction pipeline and SVM.
        End2End with hidden units $N_{h}$.
		\textbf{UAR}: Unweighted Average Recall. 
		\textbf{$r$}: Pearson's correlation coefficient.
        {\bf CSS}: COVID-19 Speech; {\bf CCS}: COVID-19 Coughing. \ls{CI for ESS \& PRS ?} \ls{Which XboX config should we use there are several for each N..?}
        \textbf{PRS}: Primates Sub-Challenge. }
% 	\vspace{0.2cm}
	\label{tab:Baselines}
\centering
%\begin{tabular}{l|rrrrrr}
%AB changed into c because right-aligned hyphens look weird
  \resizebox{\textwidth}{!}{
\begin{tabular}{l|rrrrrrrrrrr}
    \toprule
    &   \multicolumn{3}{c}{\bf CSS }    &   \multicolumn{3}{c}{\bf CCS}   &   \multicolumn{2}{c}{\bf ESS} &     \multicolumn{2}{c}{\bf PRS}     \\
    &   \multicolumn{3}{c}{UAR [\%]}  &   \multicolumn{3}{c}{UAR [\%]}     &    \multicolumn{2}{c}{UAR [\%]}     & \multicolumn{3}{c}{UAR [\%]}  \\
    \hline
    &   Dev  &   Test  & CI on Test &  Dev   & Test & CI on Test    & Dev & Test        & Dev & Test & CI on Test           \\
    \hline
    $C$             & \multicolumn{10}{c}{\bf  \textsc{openSMILE}: \textsc{ComParE}  functionals+SVM}    \\                                  
    \hline                                             
    &  57.9  &  \cellbg{72.1}  & (70.2 -- 71.1) & 61.4  & 65.5  & (66.1 - 67.2) &    70.47 & 58.60  &    82.44    &   82.21 & (78.78 -- 79.63)   \\
    
    \hline
    $N$             &   \multicolumn{10}{c}{\bf  \textsc{openXBOW}: \textsc{ComParE}  BoAW+SVM}        \\
    \hline
    $125$           &  66.0  &  63.6  & (62.0 - 63.2) & 60.7  &  66.7  & (64.5 - 65.5) & 72.18 & 55.79  & --    &   --    \\
    $250$           &  60.6  &  60.4  & (60.9 - 61.9) & 66.4  &  67.6  & (60.8 - 62.0) & 69.00 & 52.97  & 79.96    &   80.90 & (78.75 -- 79.52)    \\ %for prs 250_20
    $500$           &  64.2  &  64.7  & (62.6 - 63.7) & 66.4  &  67.5  & (65.7 - 66.8) & 70.10 & 49.39  & 83.12    &   82.43  & (80.14 -- 80.73) \\ % for prs 500_20
    $1000$          &  62.6  &  68.7  & (66.0 - 67.0) & 66.2  &  69.1  & (69.3 - 70.2) & 69.73 & 56.76 & 83.28    &   83.93  & (81.39 -- 81.85)  \\ % for prs 1000_10
    $2000$          &  66.3  &  68.7  & (64.4 - 66.4) & 64.7  &  72.9  & (71.5 - 72.2) & 70.59 & 59.80  & --    &   --    \\
    \hline
    Network         &   \multicolumn{10}{c}{\textbf{\textsc{DeepSpectrum}+SVM}}                        \\
    \hline
    DenseNet121 &   56.0 &  60.4 & (57.8 -58.7) &  63.3  &  64.1  & (65.9 - 67.1) & 64.22    &   56.38  &   81.32    &   78.82   & (76.13 -- 76.78) \\
    \hline
    $X$ [dB]        & \multicolumn{10}{c}{\bf \textsc{auDeep}: S2SAE+SVM}                            \\
    \hline
    -30             &  65.8  &  60.0  & (58.2 - 59.3) & 60.7  & 55.2  & (51.9 - 53.5) & 39.09 & 35.30 & 70.55   &   69.70 & (69.08 -- 69.53)   \\
    -45             &  66.3  &  55.2  & (54.1 - 55.2) & 64.1  & 60.5  & (61.0 - 62.0) & 41.30 & 43.07  & 80.29   &   82.26   & (80.52 -- 81.28)  \\
    -60             &  59.4  &  53.3  & (52.2 - 53.5) & 67.6  & 67.6  & (64.9 - 65.8) & 42.03 & 44.35 & 81.64   &   84.07  & (82.41 -- 83.16)  \\
    -75             &  58.4  &  52.2  & (52.0 - 52.9) & 64.0  & 64.6  & (61.0 - 62.3) & 49.02 & 52.18 & 80.67   &   82.99 & (81.50 -- 81.97)   \\
    Fused           &  62.2  &  64.2  & (62.3 - 64.2) & 65.4  & 64.2  & (62.1 - 63.1) & 46.81 & 45.02 & 84.55   &   \cellbg{86.57} & (84.57 -- 85.21)    \\
    % -30             &  65.8  &  60.0  &  61.2  & 57.3  &  --   &   --    \\
    % -45             &  66.3  &  55.2  &  60.0  & 55.8  &  --   &   --    \\
    % -60             &  59.4  &  53.3  &  60.9  & 57.8  &  --   &   --    \\
    % -75             &  58.4  &  52.2  &  57.4  & 50.1  &  --   &   --    \\
    % Fused           &  62.2  &  64.2  &  59.3  & 53.2  &  --   &   --    \\
    \hline
    Features           & \multicolumn{10}{c}{\textbf{ \textsc{DiFE}: Transformer+SVM}}                  \\
    \hline
    plain            &   --      &   -- &      --      &   --      &   --      &   --  & 51.23 & 36.81 &  --      &   --\\
    plain-BlAtt          &   --      &   -- &       --      &   --      &   --      &   --  &   50.25 &  45.16 &     &   -- \\
    sent      &   --   &    --      &   --      &   --      &   --  &   --      &   56.50 & 44.12 &  --      &   --\\
    sent-BlAtt &   --      &   -- &      --      &   --      &   --      &   --  & 47.30 & 47.19 &  --      &   --\\
    tuned-BlAtt &   --      &   -- &      --      &   --      &   --      &   --  & 43.50 & 44.93 &  --      &   --\\
%    Fused         &   --      &   -- &       --      &   --      &   --      &   --  &   --      &   -- \\
    \hline
    $N_{h}$ RNN     & \multicolumn{8}{c}{\textbf{End2End: CNN+LSTM RNN}}                            \\
    \hline
    128             & 70.5  & 68.7 & -- & 61.8 & 64.7  & -- & 64.09 &  53.98 &  72.70      &   70.80  \\
    \hline
    & \multicolumn{8}{c}{\bf {Fusion of Best}}                                                                      \\
    \hline
    &   --          & 71.1  & -- &   --          &   \cellbg{73.9}  & -- &  --  & \cellbg{59.92} &  --      &   \cellbg{--}   \\   
    %Maj.\ Vote/Mean            &      --           &   --          &   --              &  0.621        &     --       &       --      \\  
\bottomrule
\end{tabular}
}
% s\vspace{-0.5cm}
\end{table*}
